Peace in the Face of Uncertainty: Resource Allocation with Stochastic Armaments

This paper examines a government's strategic resource allocation choices when facing an opposing group whose military power is uncertain. We investigate how this uncertainty affects the government's decision to divide resources in a way that either guarantees peace, despite unresolved uncertainty, or risks conflict. We find that under low uncertainty, the government prefers distributions which ensure peace, while under high uncertainty, they are willing to risk war. When uncertainty is low, the government's allocation is decreasing in uncertainty. When uncertainty is high it is increasing. The latter leads to an increased probability of fighting and falling total welfare.

==> 0.Feedback.tex <==
\subsection{Viva}
\begin{itemize}
	\item Wanted to know when they will choose the peace guaranteeing splits and when they will risk war
	\item Asked about why it is a one-shot game (costly to negotiate,)
	\item Worried about the assumption about $\alpha>\beta>1-\alpha$
\end{itemize}

\subsection{Micro Mini Conference}
\begin{itemize}
	\item In the scenario where agents choose conflict capacity, will they not choose it in such a way as to avoid war?- so in this way might have assumed away their capacity to avoid war: this is why the model generates open conflict so easily (could be that agents have an incorrect prior about a before)
	\item Social planner's problem: eg. wants to avoid inequality, minimise the probability of war (what would minimise the probability of war in the situation where uncertainty is so large that the set of peace guaranteeing solutions is empty- interesting question)
	\item Lots of debate about the application of my model
\end{itemize}

\subsection{Discussion with Laura}
\begin{itemize}
	\item Shock can be justified by the collective action problem
	\item Acemoglu 2000 why did the west extend the franchise; Connely and Temini; Beukes; 
	\item Paper by Alesina which looks at uncertainty and macroeconomic factors [theory backs this up]
\end{itemize}


==> 4.1.Results_proofs_out.tex <==







\begin{comment}
    We direct our focus to the second case, where the likelihood of war can be controlled by flexing more benign choice variables such as the relative difference in participants' arms, as well as the proposed transfers to the rebel group. In general, however, we would not expect the destructiveness of war to be a policy tool which is easily flexed.  This is because the destructiveness of war should depend on an array of complicated factors, such as the levels of armaments controlled by belligerents, the fragility of industry in the country, and the prevalence of war crimes within the conflict.  It would be difficult for policymakers to motivate wilfully making war more destructive than it already is. This is especially true in the presence frictions such as information asymmetries about opponents' arms, or overconfidence in a decisive victory, which may result in groups accidentally engaging in an extremely destructive war.
\end{comment}
%\textbf{Possibly get rid of $t_{G}$ notation}  
\begin{comment}


Because the game is a threshold game, we have that the probability of fighting depends on the probability of the shock $\epsilon_{R}$ being above or below a particular value- thus in general we would expect the incidence of fighting to depend on the \todo{Add in some small comparative static result on the distribution of shocks}distribution of shocks.  Formally, we have that for a given value of  $\beta$, fixed in the first stage of the game, each group's probability of fighting is given by
\begin{align*}
	\mathbb{P}(BR_{G}(\epsilon_{R}) = 1) &= \begin{cases}
		0 & \text{ if } t_{G} < \underline{a} ;\\
		F_{\epsilon_{R}}\left( t_{G}\right)  & \text{ if } \underline{a} \leq t_{G}  \leq \overline{a} ;\\
		1 &\text{ if } t_{G}>\overline{a}.
	\end{cases}\\
	\mathbb{P}(BR_{R}(\epsilon_{R}) = 1) &= \begin{cases}
		0 & \text{ if } t_{R} >\overline{a};\\
		1-F_{\epsilon_{R}}\left(t_{R}\right)  & \text{ if } \underline{a} \leq t_{R}  \leq \overline{a};\\
		1 &\text{ if }\underline{a}>t_{R}.
	\end{cases}
\end{align*}
where $F_{\epsilon_{R}}$ is the CDF of $\epsilon_{R}$.
\end{comment}



 


We may, in fact, find closed form solutions for these thresholds, which readily leads to the following comparative statics:
\begin{comment}
  
\end{comment}




\begin{comment}
   As can be seen in \Cref{fig:beta_part} above, as $\beta$ increases the probability of war varies. When $\beta$ is too small to appease the government then there is always at least some risk of conflict breaking out.  fighting always occurs as the government will always reject the proposed split and attempt to repress the rebels instead. When $\beta$ increases past ${\beta_{G}}^{-}$ fighting depends on the realisation of $\epsilon_{R}$: the government will declare war of $\epsilon_{R}$ is sufficiently small. A further increase in $\beta$ then allows the government to be appeased past ${\beta_{G}}^{+}$, whilst still simultaneously appeasing the rebels. This is the set of peace-guaranteeing transfers. Finally, as $\beta$ becomes too large, the rebels can no longer be appeased and war comes back onto the table. Eventually, $\beta$ becomes too large and the rebels will always reject the proposed transfer. We illustrate this partition of $\beta$ \Cref{fig:beta_part} below.\todo{Possibly move this entire discussion and figure to section above} 
\end{comment}

 












\Cref{thm:peace_threshold} and its Corollaries describe a scenario where uncertainty in conflict capacity can be a major obstacle to negotiating peace, even in a situation where agents are equally armed. Uncertainty acts to erode agents' trust in the proposed splits of resources and thus hinders their ability to negotiate a resolution. Therefore it is not necessarily the prevalence of guns which can spark open conflict, but instead uncertainty in whether or not these guns will be useful after shocks are realised.

These results may explain why conflict is so difficult to resolve in parts of the world where military alliances are informal and the levels of armaments of each group are subject to shocks. If we look at in the developed world we see countries with large, but organized and consistent, armies, yet very little open conflict. This certainty in levels of armament could allow these countries to make deals which they know will be honoured as it is unlikely that a shock will not disrupt either party's ability to enforce the split. However, in developing countries with uncertain conflict capacities, the opposite is true: no matter how egalitarian the split of resources, the potential for a positive shock to spark a minority rebellion or a negative shock to lead to repression by the state means that even the most egalitarian institutions can be ineffective in keeping the peace.

\subsection{Comparative Statics}






Our analysis critically depends on whether the uncertainty is above or below $a_{crit}$.  If $a$ is below $a_{crit}$ then the government can propose splits that ensure peace and guarantee itself the proposed payoff $\beta$. However, if $a$ is above $a_{crit}$ then the government must risk war regardless of its proposed value of $\beta$. We therefore analyse each case separately. 

Each case leads to starkly different behaviour. When $a<a_{crit}$ the government may, under certain conditions on $\expyg-\expyr$,  guard against war by choosing a more egalitarian split of resources. However, when $a>a_{crit}$, the government abandons all attempts at negotiating peace and instead opts for highly unequal splits of $\beta$.


\subsubsection{Optimal $\beta$ when $a<a_{crit}$}



\todo{Put in plot of expected payoff function}



\begin{thm}\label{thm:optimal_beta}
	Suppose that $a<a_{crit}$, and $\alpha<1$.  Then the optimal value of the proposed transfer, $\beta^{*}$ is in $\left[{\beta_{R}}^{-}, {\beta_{R}}^{+}\right)$. Thus the government chooses a value of $\beta$ which they will always accept, but that is not so high that the rebels declare war with certainty.
\end{thm}


Notice that the pay-off function for the government at the first stage of the game is therefore piece-wise continuous on $[0,1]$.
\begin{thm}\label{prop:beta_unique}
   
\end{thm}
 
 \Cref{prop:beta_unique}
 
\begin{thm}\label{thm:risk_war}
    The government switches from guaranteeing peace to risking war as $a$ increases. As $a$ increases, the government switches from choosing to guarantee peace: $\beta^{*} = {\beta_{R}}^{-}$, to risking war: $\beta^{*} \in \left({\beta_{R}}^{-},{\beta_{R}}^{+}\right)$.\todo{Check that proof listed below actually proves this}
\end{thm}

%\begin{thm}\label{thm:risk_war}
%	There exist equilibria in which the government does not choose to guarantee peace (i.e. they risk war). Formally $\exists \beta^{*}$ in $\left({\beta_{R}}^{-},{\beta_{R}}^{+}\right)$. There exists an interval $[\underline{y},\overline{y}]$ for $\expyg-\expyr$ for which this is true.
%\end{thm}




 However, note that this second switch is not always possible for,\footnote{In particular when $\alpha$ is high.} it will be impossible for $a$ to be simultaneously larger than $\expyg-\expyr$ but smaller than $a_{crit}$, which is required for peace-guaranteeing transfers to exist.

The intuition for the return to peace-guaranteeing transfers comes from the interaction between the likelihood of war (which is increasing in $\beta$) and the probability of winning (which is decreasing in $a$ because only the rebels declare war). We have that when the government risks war, their choice of $\beta$ is increasing in $a$- thus war becomes increasingly likely as uncertainty increases. Since war is very destructive, at a certain stage it becomes too likely and the government's preference switches back to appeasement. 

In particular, we believe that this result may help describe a scenario where two countries are negotiating about nuclear disarmament, but one country has a much weaker military but their willingness to use their nuclear arms is extremely unpredictable. This may occur, for example, due to leadership by an unstable autocrat or some sort of ideological zealotry. The other country, with the larger military, has many checks and balances in place and can therefore be trusted to not suddenly launch a nuclear attack. The presence of nuclear armaments would mean that war would be very destructive (so that $\alpha$ is small relative to $\expyg-\expyr$) but uncertainty is very large relative to the difference in two countries' arms (so that $a>\expyg-\expyr$). Then, although the predictable country may still choose to offer allowances and benefits to the unstable one to prevent a nuclear war, despite having a much larger expected military capacity. This may explain, for instance, the perception that the Obama administration was quite lenient in its sanction reductions during the negotiations of the Iranian nuclear deal of 2015.

Notice that, when the second switch occurs there is an an additional policy intervention in the face of uncertainty would be to make war very destructive so that as uncertainty grows the government switches back to peace-guaranteeing transfers. However, as we discussed in the introduction, making war in developing countries even more destructive may be a politically unpopular policy. 

\Cref{thm:risk_war} shows how substantial uncertainty, by reducing the government's incentives to choose a peace-guaranteeing transfer, can be extremely detrimental to lasting peace. 

The comparative static result below gives another reason why reducing uncertainty may be desirable: increasing uncertainty drives inter-group inequality. As discussed in the introduction, inter-group inequality is often a predictive factor for war. 

\begin{prop}\label{prop:beta_deriv_a}
	Suppose that $\beta^{*} \in \left({\beta_{R}}^{-},{\beta_{R}}^{+}\right)$. Then increasing uncertainty drives increasing inequality. Formally $\beta^{*}$ is increasing in $a$. 
\end{prop}

 \Cref{prop:beta_deriv_a} states that once the government abandons the choice of peace-guaranteeing transfers it chooses to allocate an increasing share of resources to itself. The intuition for this is that since the commitment problem is so large, war becomes increasingly likely and so the government's choice to increase $\beta$ does not make a large difference to the marginal probability of war. This result paints a bleak picture of intergroup equality in the face of uncertainty and suggests that in countries where there is a large amount of conflict uncertainty we should see extremely unequal divisions of resources between groups before conflict breaks out. This matches the findings in the empirical literature.
 
 \Cref{prop:beta_deriv_a}, combined with \Cref{thm:risk_war} and the comparative statics on ${\beta_{R}}^{-}$ in \Cref{cor:beta_vals} tells us that the government's strategy switch creates a non-monotonicity in $\beta$. 
 \begin{cor}\label{cor:non-mono}
     The government's choice of $\beta^{*}$ demonstrates a non-monotonicity in $a$. In particular, when $a$ is sufficiently small so that $\beta^{*} = {\beta_{R}}^{-}$ then $\beta^{*}$ is decreasing in $a$. When $a$ is large enough so that $\beta^{*} \in \left({\beta_{R}}^{-},{\beta_{R}}^{+}\right)$ is increasing in $a$.
 \end{cor}

\begin{comment}
  \begin{prop}
	Comparative statics: payoff is always decreasing in $a$.\todo[result]{fill this in} + what happens to welfare when a peace-gauranteeing solution is chosen?
\end{prop}

\begin{proof}
	Drop in calculations from sympy?
	
	Total welfare is prob(peace)+alphaprob(war): one is increasing in a and one is decreasing in a
\end{proof}  
\end{comment}



\subsubsection{Solving for $\beta^{*}$ numerically when $a<a_{crit}$}
Categorising the exact form of the equilibrium in $\left({\beta_{R}}^{-}, {\beta_{R}}^{+}\right)$ is unfortunately a somewhat intractable exercise. It requires us to solve the first order condition
\begin{equation}\label{eq:beta_FOC}
	\frac{\alpha \beta}{{\left(1-\beta \right) \left(1-\alpha -\beta\right)}} + \frac{\alpha}{(1-\beta)} + a + y_{1} - y_{2} - \log{\left(\frac{1- \alpha - \beta}{\beta - 1} \right)}=0,
\end{equation}
on the range $\left({\beta_{R}}^{-}, {\beta_{R}}^{+}\right)$. \Cref{eq:beta_FOC} has no closed-form solutions, in general. However, the results from numerically finding the equilibrium value of $\beta^{*}$ suggest that the equilibrium value for $\beta^{*}$ is unique for all $a$ in $(0,a_{crit})$ except for a single point $\tilde{a}$, where there are two equilibria. At the point $\tilde{a}$, the government is indifferent between choosing a $\beta = {\beta_{R}}^{-}$, which guarantees peace, and $\beta^{*}>{\beta_{R}}^{-}$, which will risk war.   


Because solving for the exact equilibrium is difficult, we now turn to some simulations to solve for the optimal value of $\beta_{*}$ on $\left[{\beta_{R}}^{-},{\beta_{R}}^{+}\right)$. Our numerical solutions reveal some interesting insights.  Note that for each numerical solution, we have solved for $a$ on the entire range of possible $a$ such that $a<a_{crit}$. Our model breaks down at $a=0$, so we solve on $[10^{-4},a_{crit}]$

As shown in \Cref{cor:non-mono}, $\beta^{*}$ demonstrates a non-monotonicity in $a$: for low values of $a$ it is decreasing, and for high values of $a$ it is increasing. For low $a$ the government ensures peace. For high $a$ the government risks war. The monotonicity in $\beta^{*}$ is illustrated in \Cref{fig:beta_non_mono} below:\todo{Re-label figures}
\begin{figure}[h]
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_1_alpha_0.5.png}
		\caption{$\beta^{*} = {\beta_{R}}^{-}$ for all uncertainty}
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_1_alpha_0.7.png}
		\caption{$\beta^{*}$ demonstrates the non-monotonicity}
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_1_alpha_0.9.png}
		\caption{$\beta^{*}$ demonstrates the non-monotonicity}
	\end{subfigure}
	\hfill
	\caption{As uncertainty increases, the government switches from ensuring peace with $\beta^{*} = \beta^{2}$ to risking war with $\beta^{*}> {\beta_{R}}^{-}$.}\label{fig:beta_non_mono}
\end{figure}

From our results above, if $a>\expyg-\expyr$ then there may be a single value of $a$ at which the equilibrium is non-unique. Specifically, this may occur for certain combinations of $\alpha$ and $\expyg-\expyr$\footnote{Seemingly when $\alpha$ is small relative to $\expyg-\expyr$.}. Our simulations show that this occurs at the point where the second preference switch happens when $a$ increases. It can be seen in the jump-discontinuity in \Cref{fig:beta_switch} below.

\begin{rem}
	There exists a range of $[\underline{a},\overline{a}]$ wherein the government risks war, outside of this range the government chooses to guarantee peace.  
\end{rem}

\begin{figure}[h]
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_2.5_alpha_0.5.png}
		\caption{Two switches in monotonicity }
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_2.5_alpha_0.7.png}
		\caption{Single switch in monotonicity }
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_2.5_alpha_0.9.png}
		\caption{Single switch in monotonicity}
	\end{subfigure}
	\hfill
	\caption{For certain values of $\alpha$ and $\expyg-\expyr$, the government's optimal choice of $\beta$ demonstrates a jump-discontinuity}\label{fig:beta_switch}
\end{figure}

Finally, the simulations show that the government never risks war when $\expyg<\expyr$. This makes sense, as the probability the government will win any conflict in this scenario is quite low. Although this is theoretically good news for peace, the likelihood of the government having a lower level of arms in reality very low. We illustrate this phenomenon in \Cref{fig:beta_neg} below:

\begin{figure}[h]
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_-1_alpha_0.5.png}
		\caption{The government chooses ${\beta_{R}}^{-} \forall a<a_{crit}$}
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_-1_alpha_0.7.png}
		\caption{The government chooses ${\beta_{R}}^{-} \forall a<a_{crit}$}
	\end{subfigure}
	\hfill
	\begin{subfigure}
		[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{beta_opt_x_-1_alpha_0.9.png}
		\caption{The government chooses ${\beta_{R}}^{-} \forall a<a_{crit}$}
	\end{subfigure}
	\hfill
	\caption{When $\expyg-\expyr<0$, the government never risks war and always guarantees peace}\label{fig:beta_neg}
\end{figure}

\begin{rem}
	The government never risks war when $\expyg<\expyr$.
\end{rem}

\subsubsection{Optimal $\beta$ when $a>a_{crit}$}
We have thus far determined how uncertainty can erode the state's ability to negotiate a peaceful split of resources. We now move on to studying how the government will choose $\beta$ when uncertainty is so large that the peace-guaranteeing interval for $\beta$ is empty. We therefore now have that ${\beta_{G}}^{+}>{\beta_{R}}^{-}$, and so there is an interval where both groups are willing to fight, as shown in \Cref{fig:beta_part_fight} below:
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
		\draw [thick] (0,0) -- (10,0);
		\draw [thick] (0,-0.25) -- (0,0.25);
		\node[label = {[label distance = -9mm]{\textbf{0}}}] at (0,0) {};
		\draw [thick] (10,-0.25) -- (10,0.25);
		\node[label = {[label distance = -9mm]{\textbf{1}}}] at (10,0) {};
		
		\draw(1,-0.2) -- (1,0.2);
		\node[label = {[label distance = -9mm]{${\beta_{G}}^{-}$}}] at (1,0) {};
		\draw [pen colour = {cyan}, ultra thick,decorate, decoration = {calligraphic brace,mirror, amplitude =4pt}] (0,-1) -- (1,-1) node[pos = 0.5, below, cyan]{G always rejects};
		
		\draw(9,-0.2) -- (9,0.2);
		\node[label = {[label distance = -9mm]{${\beta_{R}}^{+}$}}] at (9,0) {};
		\draw [pen colour = {red}, ultra thick,decorate, decoration = {calligraphic brace, amplitude =4pt}] (9,0.5) -- (10,0.5) node[pos = 0.5, above, red]{R always rejects};
		
		\draw (2.5,-0.2) -- (2.5,0.2);
		\node[label = {[label distance = -9mm]{${\beta_{R}}^{-}$}}] at (2.5,0) {};
		\draw [pen colour = {red}, ultra thick,decorate, decoration = {calligraphic brace,mirror, amplitude =4pt}] (2.5,0.5) -- (0,0.5) node[pos = 0.5, above, red]{2 always accepts};
		
		\draw (7.5,-0.2) -- (7.5,0.2);
		\node[label = {[label distance = -9mm]{${\beta_{G}}^{+}$}}] at (7.5,0) {};
		\draw [pen colour = {cyan}, ultra thick,decorate, decoration = {calligraphic brace, amplitude =4pt}] (10,-1) -- (7.5,-1)  node[pos = 0.5, below, cyan]{2 always accepts};
		
		\draw [pen colour = {orange}, ultra thick,decorate, decoration = {calligraphic brace, amplitude =4pt}] (2.5,0.5) -- (7.5,0.5) node[pos = 0.5, above, orange]{Both groups willing to fight};
	\end{tikzpicture}
	\caption{An illustration of how the strategy space for $\beta$ is partitioned by fighting outcomes.}\label{fig:beta_part_fight}
\end{figure}

We have that expected pay-off, before $\epsilon_{R}$ is realised, is given by:\todo{Fix labels}

\begin{equation*}\label{eq:expec_pi_1_a_high}
	\mathbb{E}_{\epsilon_{R}}[u_{G}(\beta,\epsilon_{R})]=
	\begin{cases}
		&\alpha \tilde{p}_{G} \text{ if } \beta \in \left[0,{\beta_{G}}^{-}\right)\\
		& \alpha\mathbb{E}_{\epsilon_{R}}[p_{G}|t_{R}>\epsilon_{R}]\mathbb{P}(t_{R}>\epsilon_{R}) + \beta\mathbb{P}(t_{R}<\epsilon_{R}) \text{ if } \beta \in \left[{\beta_{G}}^{-},{\beta_{R}}^{-}\right)\\
		& \alpha \left\{\mathbb{P}(\epsilon_{R}< t_{G})\mathbf{E}_{\epsilon_{R}}[p_{G}|\epsilon_{R}< t_{G}] + \mathbb{P}(\epsilon_{R}> t_{R})\mathbf{E}_{\epsilon_{R}}[p_{G}|\epsilon_{R}> t_{R}]\right\} \\
		&+ \beta\mathbb{P}(t_{R}>\epsilon_{R}>t_{G}) \text{ if } \beta \in [{\beta_{R}}^{-},{\beta_{G}}^{+}]\\
		& \alpha\mathbb{E}_{\epsilon_{R}}[p_{G}|t_{R}>\epsilon_{R}]\mathbb{P}(t_{G}<\epsilon_{R}) + \beta\mathbb{P}(t_{R}<\epsilon_{R}) \text{ if } \beta \in \left({\beta_{G}}^{+},{\beta_{R}}^{+}\right]\\
		&\alpha\tilde{p}_{G} \text{ if } \beta \in \left({\beta_{R}}^{+},1\right].
	\end{cases} 
\end{equation*}

Our results for the optimal choice of $\beta^{*}$ when $a>a_{crit}$ are similar to those when $a<a_{crit}$ but where the government no longer chooses a peace-guaranteeing solution. Unfortunately, as was the case in the previous section when $\beta^{*}>{\beta_{R}}^{+}$, the outcome for inter-group inequality is rather grim. As we show in \Cref{thm:ethnic_inequality} when peaceful negotiation is not an option, the government abandons any attempt at distributing resources fairly amongst groups and instead chooses to completely discriminate against the rebels.  

\begin{thm}\label{thm:ethnic_inequality}
	When $a$ sufficiently large that peace cannot be guaranteed, the optimal value for $\beta$ is an interior solution and occurs in $\left({\beta_{R}}^{-},{\beta_{R}}^{+}\right)$. Moreover, $\beta^{*}$, and so the inequality of the proposed splits, increases with $a$.
\end{thm}

The intuition behind \Cref{thm:ethnic_inequality} is as follows. When uncertainty regarding the rebels' achievable conflict effort is high, there is no point in attempting to placate them by offering a favourable split of resources. This is again because of the commitment problem as it is unlikely that the rebels will honour it (if they receive a very positive shock), or be able to enforce it (if they receive a very negative shock). Thus expected utility for the government is maximised when they take all resources for themselves. In the case where the rebels receive a smaller shock to their conflict effort and are too weak to contest $\beta$, and in the case where open conflict occurs, the government is no worse off than they would be if they had proposed a lower split.


\begin{cor}\label{cor:rebellion}
    When $a$ is sufficiently large that peace cannot be guaranteed fighting will only occur when the rebels receive sufficiently large positive shocks.
\end{cor}


\Cref{cor:rebellion} shows that large levels of uncertainty lead to a scenario where we have intense repression of the minority identity group which is occasionally disrupted by rebellion. This could, for example, explain the cycles of ethnic repression followed by rebellion and violence which appear to mark many conflicts in the developing world.\todo{Add in welfare section: comparative statics on probability of war, what value of $\beta$ minimises likelihood of war} 

%\subsection{Uncertainty Makes Lasting Peace Difficult}
%Without third party enforcement civil wars rarely end in negotiated agreements (Warren 1997)

%Conflict as a renegotiation mechanism [there is substantial evidence that conflict recurs as a renegotiation mechanism]
%[brief discussion of our results]
